Satisfiability of Short Circuit Logic

The logical connectives typically found in programming languages are similar to their mathematical counterparts, yet different due to their short-circuit behaviour -- when evaluating them, the second argument is only evaluated if the first argument is not sufficient to determine the result. Combined with the possibility of side-effects, this creates a different type of logic called Short Circuit Logic. A greater theoretical understanding of this logic can lead to more efficient programming and faster program execution. In this thesis, formula satisfiability in the context of Short Circuit Logic is discussed. A formal definition of evaluation based on valuation algebras is presented, alongside an alternative definition based on valuation paths. The accompanying satisfiability and `path-satisfiability' are then proven to be equivalent, and an implementation of path-satisfiability is given. Although five types of valuation algebras can be discerned, there are only three corresponding types of valuation paths. From this, conclusions are drawn about satisfiability and side-effects; the manner in which side-effects alter truth values is relevant when analysing satisfiability, but the side-effects themselves are not.

==> chapter7.tex <==
\chapter{Populaire samenvatting}
\label{ch_samen}

Het vakgebied logica houdt zich bezig met waarheden en met formules. De logische formule $p \wedge q$, die als ``$p$ en $q$'' gelezen wordt, is \emph{waar} als zowel $p$ als $q$ waar is. Als we zouden weten dat $p$ niet waar is, dan kunnen we meteen concluderen dat $p \wedge q$ ook niet waar kan zijn; het bekijken of $q$ waar is of niet kunnen we overslaan.
Dit concept heet \emph{short-circuit evaluatie}.
Voor wiskundigen maakt een $q$-tje meer of minder vaak weinig verschil. Het bestuderen van grote structuren is niet veel lastiger dan van structuren met slechts een aantal elementen.
Als de uitkomsten van een probleem op kleine schaal bekend zijn, dan kunnen die met hetzelfde gemak vertaald worden naar het probleem op een veel grotere schaal.

In de wereld van de programmatuur ligt dit anders. 
Een computerprogramma dat een seconde nodig heeft om een probleem met tien elementen op te lossen, heeft voor een probleem met duizend elementen minuten en soms meerdere uren nodig.
Elke stap die genomen kan worden om het rekenwerk te verminderen, is dus welkom.
De logische operatoren \texttt{\&\&} en \texttt{||} in programmeertalen zoals C, Java en Haskell maken daarom gretig gebruik van short-circuit evaluatie.

Stel we voeren bijvoorbeeld het volgende stukje code uit:
\begin{verbatim}
if ( foo() && bar() )
{
  uvw()
}
else
{
  xyz()
}
\end{verbatim}
Als het uitvoeren van \texttt{foo()} onwaar oplevert, dan zal de computer het uitvoeren van \texttt{bar()} overslaan -- de formule `\texttt{foo() \&\& bar()}' kan immers niet meer waar zijn -- en direct doorgaan met het uitvoeren van \texttt{xyz()}.
Als we na veel testen zouden ontdekken dat \texttt{foo() \&\& bar()} \emph{nooit} waar kan zijn, dan kunnen we het gehele if-statement wel weggooien en gewoon `\texttt{xyz()}' neerzetten, want dat is korter, sneller en daarom beter.
Het kunnen beschrijven en voorspellen van het gedrag van zo'n if-statement is dus erg interessant voor informatici.

\vspace{5mm}
\emph{Short Circuit Logic} is een deelgebied van de logica en van de theoretische informatica dat zich bezighoudt met het gedrag van de operatoren \texttt{\&\&} en \texttt{||}.
Programma-functies zoals \texttt{foo()} en \texttt{bar()} worden in deze logica gerepresenteerd door `atomen' $a$ en $b$.
Een belangrijk verschil met traditionele logicas is dat we, vanwege het short-circuit gedrag, niet zeker weten welke atomen we wel en niet tegenkomen bij het evalueren van een formule.
Om dit te visualiseren, kunnen we evaluatiebomen bouwen, zoals in Figuur~\ref{voorbeeldboom}.
De groene bollen representeren atomen en de keuze om deze waar of onwaar te maken, en de blauwe vierkanten zijn de resultaten; T voor waar (`true') en F voor onwaar (`false').
Als het atoom $a$ bijvoorbeeld waar is, dan gaan we naar links en komen we er achter dat \texttt{a || !b} waar is. Als $a$ onwaar is, dan gaan we naar rechts, en moeten we ook het atoom $b$ bekijken. Vanwege de negatie (\texttt{!b}) vinden we onwaar als $b$ waar is, en waar als $b$ onwaar is.

\begin{figure}
\centering
\input{voorbeeldboom.tikz}
\caption{De evaluatieboom van de formule `\texttt{a || !b}'.}
\label{voorbeeldboom}
\end{figure}

Een ander essentieel verschil is dat atomen, net als functies in de programmatuur, bepaalde zijeffecten kunnen hebben. Als de functie \texttt{foo()} een externe variabele aanpast, en de functie \texttt{bar()} deze variable gebruikt, dan zal \texttt{foo() \&\& bar()} niet per se hetzelfde resultaat geven als \texttt{bar() \&\& foo()}.
Wat voor zijeffecten wel en niet toegestaan zijn, wordt gedefinieerd door een aantal restricties. Zo houdt `free' in dat alles mag, terwijl `static' geen zijeffecten toelaat. `Repetition-proof', `contractive' en `memorizing' zitten er tussen in; als een atoom bijvoorbeeld twee keer achter elkaar ge\"evalueerd wordt, dan staat `contractive' alleen de eerste keer een zijeffect toe.

Een van de vraagstukken in de logica is het vraagstuk van de \emph{satisfiability}: gegeven een formule, bijvoorbeeld $p \wedge q$, is er een keuze van $p$ en $q$ zodat deze formule waar wordt?
Uiteraard is $p \wedge q$ wel een heel simpel geval; het liefst zouden we formules in honderden variabelen willen bekijken.
Maar wanneer we dit vraagstuk op kleine schaal snel kunnen oplossen, kunnen we deze oplossing naar grotere formules vertalen.
Voor traditionele logicas is dit vraagstuk al meer dan vijftig jaar onderzocht, maar Short Circuit Logic is relatief jong.
Deze scriptie onderzoekt wat satisfiability in deze logica inhoudt, en hoe het ge\"implementeerd kan worden.

Een van de belangrijkste resultaten is dat het satisfiability-vraagstuk voor Short Circuit Logic anders gesteld kan worden: gegeven een evaluatieboom, is er een geldig pad dat bovenin de boom begint en ergens onderin de boom in een T-blad eindigt?
Met `geldig' bedoelen we hier het volgende: voor `free' is elk pad geldig, maar als in een `repetition-proof' pad twee keer achter elkaar hetzelfde atoom voorkomt, dan moet dit atoom twee keer dezelfde richting opgaan; hetzij twee keer links, hetzij twee keer rechts.
`Memorizing' geeft een sterkere restrictie aan op deze paden: elke keer dat een atoom voorkomt, moet het dezelfde richting opgaan.
Nu zijn er vijf niveaus in Short Circuit Logic die verschillende zijeffecten toestaan, maar slechts drie niveaus aan paden.
Een ander belangrijk resultaat is dan ook dat `repetition-proof' en `contractive' dezelfde satisfiability defini\"eren, en zo ook `memorizing' en `static'.
